Efficient Vertex-Oriented Polytopic Projection for Web-scale Applications

We consider applications involving a large set of instances of projecting points to polytopes. We develop an intuition guided by theoretical and empirical analysis to show that when these instances follow certain structures, a large majority of the projections lie on vertices of the polytopes. To do these projections efficiently we derive a vertex-oriented incremental algorithm to project a point onto any arbitrary polytope, as well as give specific algorithms to cater to simplex projection and polytopes where the unit box is cut by planes. Such settings are especially useful in web-scale applications such as optimal matching or allocation problems. Several such problems in internet marketplaces (e-commerce, ride-sharing, food delivery, professional services, advertising, etc.), can be formulated as Linear Programs (LP) with such polytope constraints that require a projection step in the overall optimization process. We show that in the very recent work, the polytopic projection is the most expensive step and our efficient projection algorithms help in gaining massive improvements in performance.

==> checklist.tex <==
\section*{Checklist}

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See \S~\ref{sec:introduction},\S\ref{sec:conclusion}}
  \item Did you describe the limitations of your work?
    \answerYes{See \S~\ref{sec:conclusion}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{The work can have strong positive social impact which we highlight in \S\ref{sec:conclusion}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{We follow the guidelines.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See \S~\ref{sec:projection}}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{See Appendix~\ref{app:projection}}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{Code is open sourced, we omit URL for anonymity. The instructions to reproduce results on a public-domain dataset (MovieLens) is part of the open source repository. We will reveal the link upon acceptance.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerNA{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{The problems are convex so multiple runs do not change the final solution. The variance in run times is only attributed to delays in hardware allocation in the compute cluster that affects treatment and control equally.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Section~\ref{sec:conclusion}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See \S~\ref{sec:problem}}
  \item Did you mention the license of the assets?
    \answerYes{See \S~\ref{sec:problem}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{Code is open sourced, we omit the URL in the review for anonymity.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{All data used is either public domain or respects GDPR}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{No personally identifiable information or offensive content is present in the data.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> definitions.tex <==
\RequirePackage{latexsym}
%\RequirePackage{amsmath}
% \RequirePackage{amsthm}
%\RequirePackage{amssymb}
\RequirePackage{bm}

%%%%%%%% Stock standard definitions %%%%%%%%%%%%%%%

\newcommand{\ab}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\cbb}{\mathbf{c}}
\newcommand{\db}{\mathbf{d}}
\newcommand{\eb}{\mathbf{e}}
\newcommand{\fb}{\mathbf{f}}
\newcommand{\gb}{\mathbf{g}}
\newcommand{\hb}{\mathbf{h}}
\newcommand{\ib}{\mathbf{i}}
\newcommand{\jb}{\mathbf{j}}
\newcommand{\kb}{\mathbf{k}}
\newcommand{\lb}{\mathbf{l}}
\newcommand{\mb}{\mathbf{m}}
\newcommand{\nbb}{\mathbf{n}}
\newcommand{\ob}{\mathbf{o}}
\newcommand{\pb}{\mathbf{p}}
\newcommand{\qb}{\mathbf{q}}
\newcommand{\rb}{\mathbf{r}}
\newcommand{\sbb}{\mathbf{s}}
\newcommand{\tb}{\mathbf{t}}
\newcommand{\ub}{\mathbf{u}}
\newcommand{\vb}{\mathbf{v}}
\newcommand{\wb}{\mathbf{w}}
\newcommand{\xb}{\mathbf{x}}
\newcommand{\yb}{\mathbf{y}}
\newcommand{\zb}{\mathbf{z}}

\newcommand{\abtil}{\tilde{\ab}}
\newcommand{\bbtil}{\tilde{\bb}}
\newcommand{\cbtil}{\tilde{\cbb}}
\newcommand{\dbtil}{\tilde{\db}}
\newcommand{\ebtil}{\tilde{\eb}}
\newcommand{\fbtil}{\tilde{\fb}}
\newcommand{\gbtil}{\tilde{\gb}}
\newcommand{\hbtil}{\tilde{\hb}}
\newcommand{\ibtil}{\tilde{\ib}}
\newcommand{\jbtil}{\tilde{\jb}}
\newcommand{\kbtil}{\tilde{\kb}}
\newcommand{\lbtil}{\tilde{\lb}}
\newcommand{\mbtil}{\tilde{\mb}}
\newcommand{\nbtil}{\tilde{\nbb}}
\newcommand{\obtil}{\tilde{\ob}}
\newcommand{\pbtil}{\tilde{\pb}}
\newcommand{\qbtil}{\tilde{\qb}}
\newcommand{\rbtil}{\tilde{\rb}}
\newcommand{\sbtil}{\tilde{\sbb}}
\newcommand{\tbtil}{\tilde{\tb}}
\newcommand{\ubtil}{\tilde{\ub}}
\newcommand{\vbtil}{\tilde{\vb}}
\newcommand{\wbtil}{\tilde{\wb}}
\newcommand{\xbtil}{\tilde{\xb}}
\newcommand{\ybtil}{\tilde{\yb}}
\newcommand{\zbtil}{\tilde{\zb}}

\newcommand{\atil}{\tilde{a}}
\newcommand{\btil}{\tilde{b}}
\newcommand{\ctil}{\tilde{c}}
\newcommand{\dtil}{\tilde{d}}
\newcommand{\etil}{\tilde{e}}
\newcommand{\ftil}{\tilde{f}}
\newcommand{\gtil}{\tilde{g}}
\newcommand{\htil}{\tilde{h}}
\newcommand{\itil}{\tilde{i}}
\newcommand{\jtil}{\tilde{j}}
\newcommand{\ktil}{\tilde{k}}
\newcommand{\ltil}{\tilde{l}}
\newcommand{\mtil}{\tilde{m}}
\newcommand{\ntil}{\tilde{n}}
\newcommand{\otil}{\tilde{o}}
\newcommand{\ptil}{\tilde{p}}
\newcommand{\qtil}{\tilde{q}}
\newcommand{\rtil}{\tilde{r}}
\newcommand{\stil}{\tilde{s}}
\newcommand{\ttil}{\tilde{t}}
\newcommand{\util}{\tilde{u}}
\newcommand{\vtil}{\tilde{v}}
\newcommand{\wtil}{\tilde{w}}
\newcommand{\xtil}{\tilde{x}}
\newcommand{\ytil}{\tilde{y}}
\newcommand{\ztil}{\tilde{z}}

\newcommand{\ahat}{\hat{a}}
\newcommand{\bhat}{\hat{b}}
\newcommand{\chat}{\hat{c}}
\newcommand{\dhat}{\hat{d}}
\newcommand{\ehat}{\hat{e}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\ghat}{\hat{g}}
\newcommand{\hhat}{\hat{h}}
\newcommand{\ihat}{\hat{i}}
\newcommand{\jhat}{\hat{j}}
\newcommand{\khat}{\hat{k}}
\newcommand{\lhat}{\hat{l}}
\newcommand{\mhat}{\hat{m}}
\newcommand{\nhat}{\hat{n}}
\newcommand{\ohat}{\hat{o}}
\newcommand{\phat}{\hat{p}}
\newcommand{\qhat}{\hat{q}}
\newcommand{\rhat}{\hat{r}}
\newcommand{\shat}{\hat{s}}
\newcommand{\that}{\hat{t}}
\newcommand{\uhat}{\hat{u}}
\newcommand{\vhat}{\hat{v}}
\newcommand{\what}{\hat{w}}
\newcommand{\xhat}{\hat{x}}
\newcommand{\yhat}{\hat{y}}
\newcommand{\zhat}{\hat{z}}

\newcommand{\abhat}{\hat{\ab}}
\newcommand{\bbhat}{\hat{\bb}}
\newcommand{\cbhat}{\hat{\cb}}
\newcommand{\dbhat}{\hat{\db}}
\newcommand{\ebhat}{\hat{\eb}}
\newcommand{\fbhat}{\hat{\fb}}
\newcommand{\gbhat}{\hat{\gb}}
\newcommand{\hbhat}{\hat{\hb}}
\newcommand{\ibhat}{\hat{\ib}}
\newcommand{\jbhat}{\hat{\jb}}
\newcommand{\kbhat}{\hat{\kb}}
\newcommand{\lbhat}{\hat{\lb}}
\newcommand{\mbhat}{\hat{\mb}}
\newcommand{\nbhat}{\hat{\nb}}
\newcommand{\obhat}{\hat{\ob}}
\newcommand{\pbhat}{\hat{\pb}}
\newcommand{\qbhat}{\hat{\qb}}
\newcommand{\rbhat}{\hat{\rb}}
\newcommand{\sbhat}{\hat{\sb}}
\newcommand{\tbhat}{\hat{\tb}}
\newcommand{\ubhat}{\hat{\ub}}
\newcommand{\vbhat}{\hat{\vb}}
\newcommand{\wbhat}{\hat{\wb}}
\newcommand{\xbhat}{\hat{\xb}}
\newcommand{\ybhat}{\hat{\yb}}
\newcommand{\zbhat}{\hat{\zb}}

\newcommand{\Atil}{\tilde{A}}
\newcommand{\Btil}{\tilde{B}}
\newcommand{\Ctil}{\tilde{C}}
\newcommand{\Dtil}{\tilde{D}}
\newcommand{\Etil}{\tilde{E}}
\newcommand{\Ftil}{\tilde{F}}
\newcommand{\Gtil}{\tilde{G}}
\newcommand{\Htil}{\tilde{H}}
\newcommand{\Itil}{\tilde{I}}
\newcommand{\Jtil}{\tilde{J}}
\newcommand{\Ktil}{\tilde{K}}
\newcommand{\Ltil}{\tilde{L}}
\newcommand{\Mtil}{\tilde{M}}
\newcommand{\Ntil}{\tilde{N}}
\newcommand{\Otil}{\tilde{O}}
\newcommand{\Ptil}{\tilde{P}}
\newcommand{\Qtil}{\tilde{Q}}
\newcommand{\Rtil}{\tilde{R}}
\newcommand{\Stil}{\tilde{S}}
\newcommand{\Ttil}{\tilde{T}}
\newcommand{\Util}{\tilde{U}}
\newcommand{\Vtil}{\tilde{V}}
\newcommand{\Wtil}{\tilde{W}}
\newcommand{\Xtil}{\tilde{X}}
\newcommand{\Ytil}{\tilde{Y}}
\newcommand{\Ztil}{\tilde{Z}}

\newcommand{\abar}{\bar{a}}
\newcommand{\bbar}{\bar{b}}
\newcommand{\cbar}{\bar{c}}
\newcommand{\dbar}{\bar{d}}
\newcommand{\ebar}{\bar{e}}
\newcommand{\fbar}{\bar{f}}
\newcommand{\gbar}{\bar{g}}
\newcommand{\hbr}{\bar{h}}
\newcommand{\ibar}{\bar{i}}
\newcommand{\jbar}{\bar{j}}
\newcommand{\kbar}{\bar{k}}
\newcommand{\lbar}{\bar{l}}
\newcommand{\mbar}{\bar{m}}
\newcommand{\nbar}{\bar{n}}
\newcommand{\obar}{\bar{o}}
\newcommand{\pbar}{\bar{p}}
\newcommand{\qbar}{\bar{q}}
\newcommand{\rbar}{\bar{r}}
\newcommand{\sbar}{\bar{s}}
\newcommand{\tbar}{\bar{t}}
\newcommand{\ubar}{\bar{u}}
\newcommand{\vbar}{\bar{v}}
\newcommand{\wbar}{\bar{w}}
\newcommand{\xbar}{\bar{x}}
\newcommand{\ybar}{\bar{y}}
\newcommand{\zbar}{\bar{z}}

\newcommand{\abbar}{\bar{\ab}}
\newcommand{\bbbar}{\bar{\bb}}
\newcommand{\cbbar}{\bar{\cb}}
\newcommand{\dbbar}{\bar{\db}}
\newcommand{\ebbar}{\bar{\eb}}
\newcommand{\fbbar}{\bar{\fb}}
\newcommand{\gbbar}{\bar{\gb}}
\newcommand{\hbbar}{\bar{\hb}}
\newcommand{\ibbar}{\bar{\ib}}
\newcommand{\jbbar}{\bar{\jb}}
\newcommand{\kbbar}{\bar{\kb}}
\newcommand{\lbbar}{\bar{\lb}}
\newcommand{\mbbar}{\bar{\mb}}
\newcommand{\nbbar}{\bar{\nbb}}
\newcommand{\obbar}{\bar{\ob}}
\newcommand{\pbbar}{\bar{\pb}}
\newcommand{\qbbar}{\bar{\qb}}
\newcommand{\rbbar}{\bar{\rb}}
\newcommand{\sbbar}{\bar{\sbb}}
\newcommand{\tbbar}{\bar{\tb}}
\newcommand{\ubbar}{\bar{\ub}}
\newcommand{\vbbar}{\bar{\vb}}
\newcommand{\wbbar}{\bar{\wb}}
\newcommand{\xbbar}{\bar{\xb}}
\newcommand{\ybbar}{\bar{\yb}}
\newcommand{\zbbar}{\bar{\zb}}

\newcommand{\Ab}{\mathbf{A}}
\newcommand{\Bb}{\mathbf{B}}
\newcommand{\Cb}{\mathbf{C}}
\newcommand{\Db}{\mathbf{D}}
\newcommand{\Eb}{\mathbf{E}}
\newcommand{\Fb}{\mathbf{F}}
\newcommand{\Gb}{\mathbf{G}}
\newcommand{\Hb}{\mathbf{H}}
\newcommand{\Ib}{\mathbf{I}}
\newcommand{\Jb}{\mathbf{J}}
\newcommand{\Kb}{\mathbf{K}}
\newcommand{\Lb}{\mathbf{L}}
\newcommand{\Mb}{\mathbf{M}}
\newcommand{\Nb}{\mathbf{N}}
\newcommand{\Ob}{\mathbf{O}}
\newcommand{\Pb}{\mathbf{P}}
\newcommand{\Qb}{\mathbf{Q}}
\newcommand{\Rb}{\mathbf{R}}
\newcommand{\Sbb}{\mathbf{S}}
\newcommand{\Tb}{\mathbf{T}}
\newcommand{\Ub}{\mathbf{U}}
\newcommand{\Vb}{\mathbf{V}}
\newcommand{\Wb}{\mathbf{W}}
\newcommand{\Xb}{\mathbf{X}}
\newcommand{\Yb}{\mathbf{Y}}
\newcommand{\Zb}{\mathbf{Z}}

\newcommand{\Abtil}{\tilde{\Ab}}
\newcommand{\Bbtil}{\tilde{\Bb}}
\newcommand{\Cbtil}{\tilde{\Cb}}
\newcommand{\Dbtil}{\tilde{\Db}}
\newcommand{\Ebtil}{\tilde{\Eb}}
\newcommand{\Fbtil}{\tilde{\Fb}}
\newcommand{\Gbtil}{\tilde{\Gb}}
\newcommand{\Hbtil}{\tilde{\Hb}}
\newcommand{\Ibtil}{\tilde{\Ib}}
\newcommand{\Jbtil}{\tilde{\Jb}}
\newcommand{\Kbtil}{\tilde{\Kb}}
\newcommand{\Lbtil}{\tilde{\Lb}}
\newcommand{\Mbtil}{\tilde{\Mb}}
\newcommand{\Nbtil}{\tilde{\Nb}}
\newcommand{\Obtil}{\tilde{\Ob}}
\newcommand{\Pbtil}{\tilde{\Pb}}
\newcommand{\Qbtil}{\tilde{\Qb}}
\newcommand{\Rbtil}{\tilde{\Rb}}
\newcommand{\Sbtil}{\tilde{\Sbb}}
\newcommand{\Tbtil}{\tilde{\Tb}}
\newcommand{\Ubtil}{\tilde{\Ub}}
\newcommand{\Vbtil}{\tilde{\Vb}}
\newcommand{\Wbtil}{\tilde{\Wb}}
\newcommand{\Xbtil}{\tilde{\Xb}}
\newcommand{\Ybtil}{\tilde{\Yb}}
\newcommand{\Zbtil}{\tilde{\Zb}}

\newcommand{\Abar}{\bar{A}}
\newcommand{\Bbar}{\bar{B}}
\newcommand{\Cbar}{\bar{C}}
\newcommand{\Dbar}{\bar{D}}
\newcommand{\Ebar}{\bar{E}}
\newcommand{\Fbar}{\bar{F}}
\newcommand{\Gbar}{\bar{G}}
\newcommand{\Hbar}{\bar{H}}
\newcommand{\Ibar}{\bar{I}}
\newcommand{\Jbar}{\bar{J}}
\newcommand{\Kbar}{\bar{K}}
\newcommand{\Lbar}{\bar{L}}
\newcommand{\Mbar}{\bar{M}}
\newcommand{\Nbar}{\bar{N}}
\newcommand{\Obar}{\bar{O}}
\newcommand{\Pbar}{\bar{P}}
\newcommand{\Qbar}{\bar{Q}}
\newcommand{\Rbar}{\bar{R}}
\newcommand{\Sbar}{\bar{S}}
\newcommand{\Tbar}{\bar{T}}
\newcommand{\Ubar}{\bar{U}}
\newcommand{\Vbar}{\bar{V}}
\newcommand{\Wbar}{\bar{W}}
\newcommand{\Xbar}{\bar{X}}
\newcommand{\Ybar}{\bar{Y}}
\newcommand{\Zbar}{\bar{Z}}

\newcommand{\Abbar}{\bar{\Ab}}
\newcommand{\Bbbar}{\bar{\Bb}}
\newcommand{\Cbbar}{\bar{\Cb}}
\newcommand{\Dbbar}{\bar{\Db}}
\newcommand{\Ebbar}{\bar{\Eb}}
\newcommand{\Fbbar}{\bar{\Fb}}
\newcommand{\Gbbar}{\bar{\Gb}}
\newcommand{\Hbbar}{\bar{\Hb}}
\newcommand{\Ibbar}{\bar{\Ib}}
\newcommand{\Jbbar}{\bar{\Jb}}
\newcommand{\Kbbar}{\bar{\Kb}}
\newcommand{\Lbbar}{\bar{\Lb}}
\newcommand{\Mbbar}{\bar{\Mb}}
\newcommand{\Nbbar}{\bar{\Nb}}
\newcommand{\Obbar}{\bar{\Ob}}
\newcommand{\Pbbar}{\bar{\Pb}}
\newcommand{\Qbbar}{\bar{\Qb}}
\newcommand{\Rbbar}{\bar{\Rb}}
\newcommand{\Sbbar}{\bar{\Sb}}
\newcommand{\Tbbar}{\bar{\Tb}}
\newcommand{\Ubbar}{\bar{\Ub}}
\newcommand{\Vbbar}{\bar{\Vb}}
\newcommand{\Wbbar}{\bar{\Wb}}
\newcommand{\Xbbar}{\bar{\Xb}}
\newcommand{\Ybbar}{\bar{\Yb}}
\newcommand{\Zbbar}{\bar{\Zb}}

\newcommand{\Ahat}{\hat{A}}
\newcommand{\Bhat}{\hat{B}}
\newcommand{\Chat}{\hat{C}}
\newcommand{\Dhat}{\hat{D}}
\newcommand{\Ehat}{\hat{E}}
\newcommand{\Fhat}{\hat{F}}
\newcommand{\Ghat}{\hat{G}}
\newcommand{\Hhat}{\hat{H}}
\newcommand{\Ihat}{\hat{I}}
\newcommand{\Jhat}{\hat{J}}
\newcommand{\Khat}{\hat{K}}
\newcommand{\Lhat}{\hat{L}}
\newcommand{\Mhat}{\hat{M}}
\newcommand{\Nhat}{\hat{N}}
\newcommand{\Ohat}{\hat{O}}
\newcommand{\Phat}{\hat{P}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\Rhat}{\hat{R}}
\newcommand{\Shat}{\hat{S}}
\newcommand{\That}{\hat{T}}
\newcommand{\Uhat}{\hat{U}}
\newcommand{\Vhat}{\hat{V}}
\newcommand{\What}{\hat{W}}
\newcommand{\Xhat}{\hat{X}}
\newcommand{\Yhat}{\hat{Y}}
\newcommand{\Zhat}{\hat{Z}}

\newcommand{\Abhat}{\hat{\Ab}}
\newcommand{\Bbhat}{\hat{\Bb}}
\newcommand{\Cbhat}{\hat{\Cb}}
\newcommand{\Dbhat}{\hat{\Db}}
\newcommand{\Ebhat}{\hat{\Eb}}
\newcommand{\Fbhat}{\hat{\Fb}}
\newcommand{\Gbhat}{\hat{\Gb}}
\newcommand{\Hbhat}{\hat{\Hb}}
\newcommand{\Ibhat}{\hat{\Ib}}
\newcommand{\Jbhat}{\hat{\Jb}}
\newcommand{\Kbhat}{\hat{\Kb}}
\newcommand{\Lbhat}{\hat{\Lb}}
\newcommand{\Mbhat}{\hat{\Mb}}
\newcommand{\Nbhat}{\hat{\Nb}}
\newcommand{\Obhat}{\hat{\Ob}}
\newcommand{\Pbhat}{\hat{\Pb}}
\newcommand{\Qbhat}{\hat{\Qb}}
\newcommand{\Rbhat}{\hat{\Rb}}
\newcommand{\Sbhat}{\hat{\Sb}}
\newcommand{\Tbhat}{\hat{\Tb}}
\newcommand{\Ubhat}{\hat{\Ub}}
\newcommand{\Vbhat}{\hat{\Vb}}
\newcommand{\Wbhat}{\hat{\Wb}}
\newcommand{\Xbhat}{\hat{\Xb}}
\newcommand{\Ybhat}{\hat{\Yb}}
\newcommand{\Zbhat}{\hat{\Zb}}

\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{{\mathcal{S}}}
\newcommand{\Tcal}{{\mathcal{T}}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}

\newcommand{\Atilde}{\widetilde{A}}
\newcommand{\Btilde}{\widetilde{B}}
\newcommand{\Ctilde}{\widetilde{C}}
\newcommand{\Dtilde}{\widetilde{D}}
\newcommand{\Etilde}{\widetilde{E}}
\newcommand{\Ftilde}{\widetilde{F}}
\newcommand{\Gtilde}{\widetilde{G}}
\newcommand{\Htilde}{\widetilde{H}}
\newcommand{\Itilde}{\widetilde{I}}
\newcommand{\Jtilde}{\widetilde{J}}
\newcommand{\Ktilde}{\widetilde{K}}
\newcommand{\Ltilde}{\widetilde{L}}
\newcommand{\Mtilde}{\widetilde{M}}
\newcommand{\Ntilde}{\widetilde{N}}
\newcommand{\Otilde}{\widetilde{O}}
\newcommand{\Ptilde}{\widetilde{P}}
\newcommand{\Qtilde}{\widetilde{Q}}
\newcommand{\Rtilde}{\widetilde{R}}
\newcommand{\Stilde}{\widetilde{S}}
\newcommand{\Ttilde}{\widetilde{T}}
\newcommand{\Utilde}{\widetilde{U}}
\newcommand{\Vtilde}{\widetilde{V}}
\newcommand{\Wtilde}{\widetilde{W}}
\newcommand{\Xtilde}{\widetilde{X}}
\newcommand{\Ytilde}{\widetilde{Y}}
\newcommand{\Ztilde}{\widetilde{Z}}

\renewcommand{\vec}[1]{\mathbf{\boldsymbol{#1}}}

\newcommand{\avec}{\vec{a}}
\newcommand{\bvec}{\vec{b}}
\newcommand{\cvec}{\vec{c}}
\newcommand{\dvec}{\vec{d}}
\newcommand{\evec}{\vec{e}}
\newcommand{\fvec}{\vec{f}}
\newcommand{\gvec}{\vec{g}}
\newcommand{\hvec}{\vec{h}}
\newcommand{\ivec}{\vec{i}}
\newcommand{\jvec}{\vec{j}}
\newcommand{\kvec}{\vec{k}}
\newcommand{\lvec}{\vec{l}}
\newcommand{\mvec}{\vec{m}}
\newcommand{\nvec}{\vec{n}}
\newcommand{\ovec}{\vec{o}}
\newcommand{\pvec}{\vec{p}}
\newcommand{\qvec}{\vec{q}}
\newcommand{\rvec}{\vec{r}}
\newcommand{\svec}{\vec{s}}
\newcommand{\tvec}{\vec{t}}
\newcommand{\uvec}{\vec{u}}
\newcommand{\vvec}{\vec{v}}
\newcommand{\wvec}{\vec{w}}
\newcommand{\xvec}{\vec{x}}
\newcommand{\yvec}{\vec{y}}
\newcommand{\zvec}{\vec{z}}

\newcommand{\va}{\vec{a}}
\newcommand{\vecb}{\vec{b}}
\newcommand{\vc}{\vec{c}}
\newcommand{\vd}{\vec{d}}
\newcommand{\veee}{\vec{e}}
\newcommand{\vf}{\vec{f}}
\newcommand{\vg}{\vec{g}}
\newcommand{\vh}{\vec{h}}
\newcommand{\vi}{\vec{i}}
\newcommand{\vo}{\vec{o}}
\newcommand{\vp}{\vec{p}}
\newcommand{\vq}{\vec{q}}
\newcommand{\vr}{\vec{r}}
\newcommand{\vs}{\vec{s}}
\newcommand{\vt}{\vec{t}}
\newcommand{\vu}{\vec{u}}
\newcommand{\vv}{\vec{v}}
\newcommand{\vx}{\vec{x}}
\newcommand{\vw}{\vec{w}}
\newcommand{\vy}{\vec{y}}
\newcommand{\vz}{\vec{z}}

\newcommand{\Avec}{\vec{A}}
\newcommand{\Bvec}{\vec{B}}
\newcommand{\Cvec}{\vec{C}}
\newcommand{\Dvec}{\vec{D}}
\newcommand{\Evec}{\vec{E}}
\newcommand{\Fvec}{\vec{F}}
\newcommand{\Gvec}{\vec{G}}
\newcommand{\Hvec}{\vec{H}}
\newcommand{\Ivec}{\vec{I}}
\newcommand{\Jvec}{\vec{J}}
\newcommand{\Kvec}{\vec{K}}
\newcommand{\Lvec}{\vec{L}}
\newcommand{\Mvec}{\vec{M}}
\newcommand{\Nvec}{\vec{N}}
\newcommand{\Ovec}{\vec{O}}
\newcommand{\Pvec}{\vec{P}}
\newcommand{\Qvec}{\vec{Q}}
\newcommand{\Rvec}{\vec{R}}
\newcommand{\Svec}{\vec{S}}
\newcommand{\Tvec}{\vec{T}}
\newcommand{\Uvec}{\vec{U}}
\newcommand{\Vvec}{\vec{V}}
\newcommand{\Wvec}{\vec{W}}
\newcommand{\Xvec}{\vec{X}}
\newcommand{\Yvec}{\vec{Y}}
\newcommand{\Zvec}{\vec{Z}}

\newcommand{\Amat}{\Ab}
\newcommand{\Bmat}{\Bb}
\newcommand{\Cmat}{\Cb}
\newcommand{\Dmat}{\Db}
\newcommand{\Emat}{\Eb}
\newcommand{\Fmat}{\Fb}
\newcommand{\Gmat}{\Gb}
\newcommand{\Hmat}{\Hb}
\newcommand{\Imat}{\Ib}

\newcommand{\Vmat}{\Vb}
\newcommand{\Wmat}{\Wb}
\newcommand{\Xmat}{\Xb}
\newcommand{\Ymat}{\Yb}
\newcommand{\Zmat}{\Zb}


\newcommand{\yvecbar}{\bar{\vec{y}}}
\newcommand{\wvecbar}{\bar{\vec{w}}}
\newcommand{\xvecbar}{\bar{\vec{x}}}
\newcommand{\yvectil}{\tilde{\vec{y}}}
\newcommand{\yvechat}{\hat{\vec{y}}}


%%%%%%%% Theorems and Friends %%%%%%%%%%%%%%%

%% Some style files might actually define these variables.
%% So don't mess with them if they are already defined

\ifx\BlackBox\undefined
\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\fi

\ifx\QED\undefined
\def\QED{~\rule[-1pt]{5pt}{5pt}\par\medskip}
\fi

\ifx\proof\undefined
\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}
\fi

\ifx\theorem\undefined
\newtheorem{theorem}{Theorem}
\fi

\ifx\example\undefined
\newtheorem{example}{Example}
\fi

\ifx\property\undefined
\newtheorem{property}{Property}
\fi

\ifx\lemma\undefined
\newtheorem{lemma}{Lemma}
\fi

\ifx\proposition\undefined
\newtheorem{proposition}{Proposition}
\fi

\ifx\remark\undefined
\newtheorem{remark}{Remark}
\fi

\ifx\corollary\undefined
\newtheorem{corollary}{Corollary}
\fi

\ifx\definition\undefined
\newtheorem{definition}{Definition}
\fi

\ifx\conjecture\undefined
\newtheorem{conjecture}{Conjecture}
\fi

\ifx\axiom\undefined
\newtheorem{axiom}{Axiom}
\fi

\ifx\claim\undefined
\newtheorem{claim}{Claim}
\fi

\ifx\assumption\undefined
\newtheorem{assumption}{Assumption}
\fi

% \renewcommand{\qedsymbol}{$\blacksquare$}


%%%%%%%% Widely accepted Sets and Symbols %%%%%%%%%%%%%%%

\newcommand{\CC}{\mathbb{C}} % Complex numbers
\newcommand{\EE}{\mathbb{E}} % Expectation
\newcommand{\FF}{\mathbb{F}} % Fexpectation
\newcommand{\HH}{\mathbb{H}} % Arbitrary field
\newcommand{\II}{\mathbb{I}} % Delta Indicator
\newcommand{\KK}{\mathbb{K}} % Arbitrary field
\newcommand{\MM}{\mathbb{M}} % Median
\newcommand{\NN}{\mathbb{N}} % Natural numbers
\newcommand{\PP}{\mathbb{P}} % Probability
\newcommand{\QQ}{\mathbb{Q}} % Rationals
\newcommand{\real}{\mathbb{R}} % Real numbers
\newcommand{\RRbar}{\overline{\RR}} % Real numbers
\newcommand{\VV}{\mathbb{V}} % Variance
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}} % Integers

%%%%%%%% Mathematical Operations %%%%%%%%%%%%%%%

%\newcommand*{\mini}{\mathop{\mathrm{minimize}}}
%\newcommand*{\maxi}{\mathop{\mathrm{maximize}}}
\newcommand*{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand*{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand*{\arginf}{\mathop{\mathrm{arginf}}}
\newcommand*{\argsup}{\mathop{\mathrm{argsup}}}
\newcommand{\sgn}{\mathop{\mathrm{sign}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\diag}{\mathop{\mathrm{diag}}}
\newcommand{\rank}{\mathop{\mathrm{rank}}}
\newcommand{\vect}{\mathop{\mathrm{vec}}}
\newcommand{\traj}{\mathop{\mathrm{Traj}}}
\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\const}{\mathrm{constant}}
\newcommand{\dom}{\mathop{\mathrm{dom}}}
\newcommand{\ri}{\mathop{\mathrm{ri}}}
\newcommand{\cl}{\mathop{\mathrm{cl}}}
\newcommand{\intr}{\mathop{\mathrm{int}}}
\newcommand{\bd}{\mathop{\mathrm{bd}}}
\newcommand{\emp}{\mathop{\mathrm{emp}}}
\newcommand{\core}{\mathop{\mathrm{core}}}
\newcommand{\co}{\mathop{\mathrm{co}}}
\newcommand{\nnz}{\mathop{\mathrm{nnz}}}
\newcommand{\eproof}{$\null\hfill\blacksquare$}

%\newcommand{\ln}{\mathop{\mathrm{ln}}}
%%%%%%%% Utility functions %%%%%%%%%%%%%%%

\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}
\newcommand{\mychoose}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\newcommand{\mydet}[1]{\det\left[ #1 \right]}
\newcommand{\myspan}[1]{\mathrm{span}\cbr{#1}}
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}
\newcommand{\pwrt}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ppwrt}[1]{\frac{\partial^2}{(\partial #1)^2}}
\newcommand{\aleq}{\preccurlyeq}
\newcommand{\ageq}{\succcurlyeq}
%%%%%%%% Short Forms %%%%%%%%%%%%%%%

\newcommand{\ea}{\emph{et al.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\iid}{\emph{iid}}
\newcommand{\cf}{\emph{cf.}\ }
\newcommand{\wrt}{\emph{w.r.t.}\ }

%%%%%%%% Brackets %%%%%%%%%%%%%%%

\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\ccc}[1]{|\!|\!|#1|\!|\!|}
\newcommand{\cccc}[1]{\left|\!\left|\!\left|#1\right|\!\right|\!\right|}
\newcommand{\sembrack}[1]{[\![#1]\!]}

%%%%%%%%%%%%%%%  Mathematical Constants  %%%%%%%%%%%%%%%

\newcommand{\one}{\mathbf{1}}  % Identity
\newcommand{\zero}{\mathbf{0}} % Zero
\newcommand{\ind}{\boldsymbol{\mathsf{I}}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\sqrttwo}{\sqrt{2}}
\newcommand{\invsqrttwo}{\frac{1}{\sqrt{2}}}
\newcommand{\rmd}{\ensuremath{\mathrm{d}}}

%%%%%%%% Greek Symbols %%%%%%%%%%%%%%%

\newcommand{\sigmab}{\bm{\sigma}}
\newcommand{\Sigmab}{\mathbf{\Sigma}}

\newcommand{\val}{\vec{\alpha}}
\newcommand{\vbeta}{\vec{\beta}}
\newcommand{\vde}{\vec{\delta}}
\newcommand{\vga}{\vec{\gamma}}
\newcommand{\vsig}{\vec{\sigma}}
\newcommand{\vth}{\vec{\theta}}
\newcommand{\veta}{\vec{\eta}}
\newcommand{\vnu}{\vec{\nu}}
\newcommand{\vpsi}{\vec{\psi}}
\newcommand{\vpi}{\vec{\pi}}
\newcommand{\vphi}{\vec{\phi}}
\newcommand{\vxi}{\vec{\xi}}
\newcommand{\vze}{\vec{\zeta}}

\newcommand{\valbar}{\bar{\val}}
\newcommand{\valhat}{\hat{\val}}
\newcommand{\valtil}{\tilde{\val}}
\newcommand{\vthtil}{\tilde{\vth}}
\newcommand{\vthhat}{\hat{\vth}}
\newcommand{\vthbar}{\bar{\vth}}
\newcommand{\vbetatil}{\tilde{\vbeta}}
\newcommand{\vbetahat}{\hat{\vbeta}}

\newcommand{\alphavec}{\val}
\newcommand{\alphavecbar}{\bar{\val}}
\newcommand{\alphavechat}{\hat{\val}}
\newcommand{\alphavectil}{\tilde{\val}}
\newcommand{\betavec}{\vec{\beta}}
\newcommand{\gammavec}{\vec{\gamma}}
\newcommand{\deltavec}{\vec{\delta}}
\newcommand{\etavec}{\vec{\eta}}
\newcommand{\phivec}{\vec{\phi}}
\newcommand{\psivec}{\vec{\psi}}
\newcommand{\thetavec}{\vec{\theta}}
\newcommand{\muvec}{\vec{\mu}}
\newcommand{\xivec}{\vec{\xi}}
\newcommand{\chivec}{\vec{\chi}}
\newcommand{\lambdavec}{\vec{\lambda}}

\newcommand{\alphab}{\boldsymbol{\alpha}}
\newcommand{\betab}{\boldsymbol{\beta}}
\newcommand{\gammab}{\boldsymbol{\gamma}}
\newcommand{\thetab}{\boldsymbol{\theta}}
\newcommand{\mub}{\boldsymbol{\mu}}
\newcommand{\nub}{\boldsymbol{\nu}}
\newcommand{\xib}{\boldsymbol{\xi}}
\newcommand{\Deltab}{\boldsymbol{\Delta}}
\newcommand{\Pib}{\boldsymbol{\Pi}}
\newcommand{\etab}{\boldsymbol{\eta}}
\newcommand{\taub}{\boldsymbol{\tau}}
\newcommand{\lambdab}{\boldsymbol{\lambda}}
\newcommand{\pitil}{\tilde{\pi}}
\newcommand{\elltil}{\tilde{\ell}}
\newcommand{\rhob}{\boldsymbol{\rho}}

\newcommand{\delhat}{\hat{\delta}}
\newcommand{\phihat}{\hat{\phi}}
\newcommand{\delbar}{\bar{\delta}}
\newcommand{\alphahat}{\hat{\alpha}}
\newcommand{\alphatil}{\tilde{\alpha}}
\newcommand{\mubar}{\bar{\mu}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\thetabar}{\bar{\theta}}
\newcommand{\betahat}{\hat{\beta}}

\newcommand{\xibar}{\bar{\xi}}
\newcommand{\lambdavectil}{\tilde{\vec{\lambda}}}
\newcommand{\lambdatil}{\tilde{\lambda}}
\newcommand{\lambdabar}{\bar{\lambda}}
\newcommand{\thetatil}{\tilde{\theta}}
\newcommand{\betatil}{\tilde{\beta}}

%%%%%%%% Various Optimizers %%%%%%%%%%%%%%%

\newcommand{\BMRM}{{\sf BMRM}}
\newcommand{\bmrm}{{\sf BMRM}}
\newcommand{\cpm}{{\sf CPM}}
\newcommand{\liblinear}{{\sf liblinear}}
\newcommand{\lsbmrm}{{\sf ls-bmrm}}
\newcommand{\qpbmrm}{{\sf qp-bmrm}}
\newcommand{\pegasos}{{\sf pegasos}}
\newcommand{\pegan}{{\sf pegasos-$n$}}
\newcommand{\pegaone}{{\sf pegasos-1}}
\newcommand{\svmstruct}{{\sf SVM-Struct}}
\newcommand{\svmperf}{{\sf SVM-Perf}}
\newcommand{\nest}{{\sf pragam}}
\newcommand{\nestb}{{\sf pragam-b}}
\newcommand{\mcn}{{\sf M$^3$N}}
\newcommand{\expgrad}{{\sf ExpGrad}}
\newcommand{\smo}{{\sf SMO}}
\newcommand{\lasvm}{{\sf LaSVM}}
\newcommand{\sms}{{\sf SMS}}
\newcommand{\agm}{{\sf AGM}}


\newcommand{\prbep}{{\sf PRBEP}}
\newcommand{\rocarea}{{\sf ROCArea}}

\newcommand{\arow}[2]{#1_{#2\cdot}}
\newcommand{\acol}[2]{#1_{\cdot#2}}
\newcommand{\expunder}[1]{\mathop{\EE}\limits_{#1}}
\newcommand{\mean}[1]{\mathop{\EE}\sbr{{#1}}}
\newcommand{\vars}[2]{\var_{{#1}}\sbr{{#2}}}
\newcommand{\expec}[2]{\mathop{\EE}_{{#1}}\sbr{{#2}}}

\newcommand{\twoco}[1]{\multicolumn{2}{c|}{#1}}
\def\ci{\perp\!\!\!\perp}

\newcommand{\ve}{\varepsilon}

\newcommand{\gstar}{g^{\star}}
\newcommand{\fstar}{f^{\star}}
\newcommand{\hstar}{h^{\star}}
\newcommand{\Astar}{A^{\star}}
\newcommand{\Kstar}{K^{\star}}

\newcommand{\var}{\mathrm{Var}}
\newcommand{\grad}{{\nabla}}
\newcommand{\gradtil}{{\tilde{\grad}}}
\newcommand{\MED}{{\text{MED}}}
\newcommand{\where}{{\quad \text{where} \quad}}
\newcommand{\lcg}{{\textit{l.c.g}}}
%\newcommand{\cp}{\mathrm{cp}}
\newcommand{\err}{{\sf err}}
\newcommand{\wvechat}{\hat{\vec{w}}}

\newcommand{\ydiff}[2]{\delta(#1, #2)}
\newcommand{\ykdiff}[2]{\delta(#1, #2)^{\kappa}}
\newcommand{\myfdiff}[2]{\Delta f(#1, #2)}


\newcommand{\Aone}{\textbf{A1}}
\newcommand{\Atwo}{\textbf{A2}}


==> paper/gamma.tex <==
\def\defeq{\stackrel{\text{def}}{=}}
\def\psitil{\tilde{\psi}}

\section{Adaptive Smoothing Algorithm}
\label{sec:gamma}

The smoothness of $g_\gamma$
%\footnote{We can measure smoothness in terms of the inverse of the Lipschitz constant.} 
decreases as the number of constraints  increases. %Thus treating $\gamma$ as just a hyperparameter to the optimization process is subpar since 
A small $\gamma$ makes the optimizer's convergence prohibitively slow, while a large $\gamma$ reduces the accuracy of the solution. Guided by theory, we define a practical criterion for sufficient convergence for a given $\gamma$ and describe a stage-wise algorithm that automatically reduces $\gamma$ when the criterion is met to prefer more accurate solutions. 
%We go on to empirically show that the criterion is a good proxy to the duality gap in cases where it is non trivial to compute a primal feasible solution. \keerthi{Revisit this sentence after the results are seen.}

Let $\lambda_\gamma = \arg \max_{\lambda\ge 0} g_\gamma(\lambda)$ and $\lambdatil_\gamma$ be an approximate solution after the optimizer has made sufficient progress to maximize $g_\gamma$. If the approximation error $(g_0(\lambda_0) - g_0(\lambdatil_\gamma))$ is $\epsilon$ times smaller than the total opportunity $(g_0(\lambda_0) - g_0(0))$ then we declare sufficient convergence, i.e.,
\begin{eqnarray}
    g_0(\lambda_0) - g_0(\lambdatil_\gamma) \le \epsilon \; (g_0(\lambda_0) - g_0(0)). \label{geq:eq0}
\end{eqnarray}
The intuition behind \eqref{geq:eq0} is as follows:
\begin{compactenum}
\item The criterion is defined in terms of $g_0$ because it is the Lagrangian dual corresponding to the actual LP we want to solve and by strong duality, $g_0(\lambda_0)$ is the optimal primal objective that can be attained. 
\item Since $\lambda=0$ removes the effect of constraints on the Lagrangian, $g_0(0)$ represents the maximum value of the primal objective. The total opportunity represents the value of objective ``lost'' to enforce the constraints $Ax \le b$.
\item The approximation error (the left hand side of (\ref{geq:eq0})) is due to two levels of approximation: (a) the error due to working with $\gamma >0$, i.e., the difference between $\lambda_0$ and $\lambda_\gamma$; and (b) the approximate solution of $\max_\lambda g_\gamma(\lambda)$, i.e., the difference between $\lambda_\gamma$ and $\lambdatil_\gamma$.
\end{compactenum} 

{ \bf Stage-wise adaptation of $\boldsymbol{\gamma}$: }
%\label{subsec:gammastage}
Since the true solution ($\lambda_0$) in the left hand side of (\ref{geq:eq0}) is unavailable we define an approximate bound which can be used to detect convergence. This bound is based on the following result.%lemma (proof and other details are in Appendix \ref{app:gamma} of the supplement~\cite{supplement}).

%$\xtil_0 = \xtil(\lambda_0)$ is as in (\ref{eq:xstar}),  

%\kinjal{To discuss notations}
\begin{lemma}
If $\xtil_0 = \Pi_{\mathcal{C}}[-\tfrac{1}{\gamma}(A^T\lambda_0 + c)]$ %is the projection of $\frac{1}{\gamma}(c+A^T\lambda_0)$ to $\C$,
%$\xtil_0 = \arg\min_{x \in \mathcal C} \{ c^T x + \frac{\gamma}{2} x^Tx +$ $(\lambda_0)^T(Ax-b) \}$,
then
\begin{equation}
    g_0(\lambda_0) - g_0(\lambdatil_\gamma) \le ( g_0(\lambda_\gamma) - g_0(\lambdatil_\gamma) ) + \gamma \psi(\gamma)
    \label{geq:eq1}
\end{equation}
where
%\begin{equation}
$\psi(\gamma)  = (\max_{x \in \mathcal C} \frac{1}{2} x^Tx)  - \frac{1}{2} \xtil_0^T\xtil_0$. %\label{eq:psinew}
%\end{equation}
\end{lemma} 
%and
% \begin{equation}
%     \xtil_0 = \arg\min_{x \in \mathcal C} \left\{ c^T x + \frac{\gamma}{2} x^Tx + (\lambda_0)^T(Ax-b) \right\}
% \end{equation}

Let $g_{\text{drop}} \approx (g_0(\lambda_0) - g_0(0))$ and $\psi_a \approx \psi(\gamma)$ be good practical approximations  to the corresponding true quantities and $\lambdabar_\gamma$ be the solution obtained after a fixed  number of optimization iterations are run after $\lambdatil_\gamma$ was obtained. Then using (\ref{geq:eq0}) and (\ref{geq:eq1}), 
%(details in Appendix \ref{app:gamma} of the supplement~\cite{supplement}), 
the criterion for sufficient convergence can be taken to hold if
% \begin{eqnarray}
% \gamma \psi_a \le \frac{\epsilon}{2} g_{\text{drop}} \mbox{ and } ( g_0(\lambda_\gamma) - g_0(\lambdatil_\gamma) ) \le \frac{\epsilon}{2} g_{\text{drop}} \label{eq:prac1}
% \end{eqnarray}
% Since $g_0(\lambda_\gamma)$ is an unknown quantity, we can replace it with $g_0(\lambdabar_\gamma)$ where $\lambdabar_\gamma$ is a point that comes some $K$ iterations after $\lambdatil_\gamma$ was computed.\footnote{The larger $K$ is, the better is the approximation that goes from (\ref{eq:prac1}) to (\ref{eq:prac2}).} Thus, we replace (\ref{eq:prac1}) by
\begin{eqnarray}
 ( g_0(\lambdabar_\gamma) - g_0(\lambdatil_\gamma) ) \le \frac{\epsilon}{2} g_{\text{drop}} \mbox{ and } \gamma \psi_a \le \frac{\epsilon}{2} g_{\text{drop}} \label{geq:prac}
\end{eqnarray}
This forms the backbone of our adaptive smoothness algorithm. In practice, $\epsilon=10^{-3}$ works well in recovering the optimal solution. The idea is to do three stages, trying three decreasing values of $\gamma$, with $\epsilon$ changing as $10^{-t}$, $t=1,2,3$. In each stage we pick $\epsilon$ and use the second condition in (\ref{geq:prac}) to select $\gamma$ and run the optimizer until the first condition is satisfied. As already mentioned, the reason for working with larger $\epsilon$ values in the earlier stages is to work with a smoother objective so that gradient based optimization algorithms work more effectively. 
%(see Appendix \ref{app:gamma} for details).

\textbf{Caveat:} The above definition of $\psi_a$ depends on $\gamma$. To pick the first value of $\gamma$ we bound $\psi_a$ using the information about the projection being used. If $\Itil$ is the number of vertex minimizers in $\xtil_0$, then $\xtil_0^T\xtil_0 \ge \Itil \delta$, where $\delta=1$ for {\it Simplex-E(I)} and $1 < \delta < K$ for {\it Box-Cut-E(I)}. Also, $\max_{x \in \mathcal C} \frac{1}{2} x^Tx \le \delta I$. By Theorem \ref{thm:corral}, $(I-\Itil) \ge m$. Using these it follows that 
$\psi(\gamma) \le m\delta/2 \defeq \psitil$.
%\begin{equation}
%    \psi(\gamma) \le \frac{1}{2} m\delta \defeq \psitil %\label{geq:sard}
%\end{equation}
Thus, $\psitil$ is not only a good approximation to $\psi_a$ but it is also independent of $\gamma$. Although $\psitil$ is based on analysis at $\gamma=0$, we find in our experimentation that $\Itil$ at $\gamma > 0$ is not too different from $\Itil$ at $\gamma=0$.

{\bf Approximating $\boldsymbol{g_{\text{drop}}}$: }
%\label{subsec:gammagdrop}
At stage $t$, we use the best known solution so far, i.e. $\lambdabar_\gamma \approx \lambda_0$ from stage $t-1$, to compute $g_{\text{drop}}$ and $\psi_a$. We find this to work well in practice. In the first stage, we approximate $g_{\text{drop}} \approx \tau |g_0(0)|$, where $\tau$ represents the user's estimate of of $(g_0(\lambda_0) - g_0(0))$ as a fraction of $|g_0(0)|$. When unknown, setting $\tau=1$ works well since the first stage uses a crude tolerance $\epsilon=10^{-1}$ and the first $\gamma$ choice is not crucial; the algorithm will become more cautious when choosing the subsequent $\gamma$ values in the second and third stages.

%\keerthi{I will rewrite the part below after the results are inserted.}

%{\bf How good is the sufficient convergence criterion? }
%\label{subsec:gammasuff}
%For web-scale matching problems using a subset of the projections, i.e. {\it I} variants, we can compute $\hat{x}_{feasible} = \delta \hat{x}$. $\delta = (\delta_1, ... , \delta_j)$ where $\delta_j = b_j/ax_j$. The primal objective is calculated as $c*\hat{x}_{feasible}$ and the dual objective is $g_0(\lambda)$.
%The duality gap is
%\begin{align*}
%    \frac{|\text{primalObj}_t - \text{dualObj}_t|}{1 + 0.5|\text{primalObj}_t| + 0.5|\text{dualObj}_t|} < \epsilon
%\end{align*}
%Now, we can compare both the stopping criteria.

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.15]{img/gamma.png}
    %\vspace{-0.2cm}
    \caption{The effect of smoothness of $g_\gamma$ on $Q(\lambda)$ in dataset $D_2$. $Q$ denotes solution quality; see \S\ref{sec:experiments} and (\ref{eq:quality}) for its definition.}
    \label{fig:gamma-results}
%\vskip -0.1in
\end{figure}

The choice of $\gamma$ changes the smoothness of $g_\gamma$ thereby influencing the speed of convergence. A large $\gamma$ (blue curve in Figure \ref{fig:gamma-results}) will help the optimizer make progress quickly but will hit a poor plateau 
on $g_0$.
%beyond which $\lambda$ cannot improve. 
Conversely, a small $\gamma$ (green curve in Figure \ref{fig:gamma-results}) will 
%will consistently improve $g_{\gamma}$ 
reach a very good final $g_0$ value, but the progress will be too slow. 
%Although, one could use techniques like grid-search to find the 
The largest $\gamma$ that reaches the needed accuracy on $g_0$ is dataset-dependent. 
%each dataset typically has a different sensitivity to $\gamma$ making this a hard problem. 
Our algorithm automatically adapts $\gamma$ in three stages to handle the speed-accuracy tradeoff
%allowing the optimizer to make progress quickly 
without any manual tuning. 
%As we get close to the true solution, the algorithm picks a small $\gamma$ allowing the solver to compute more accurate solutions. 
This is seen on all datasets (\S\ref{subsec:applications}); we show this %for one dataset 
in Figure~\ref{fig:gamma-results}.


==> paper/optim.tex <==

\section{Optimization}
\label{sec:optimization}

In \S\ref{sec:projection}, we focused on speeding up one evaluation of $(g_\gamma, \nabla g_\gamma)$ by making the inner projection steps very efficient. An orthogonal way of speeding up the solution of (\ref{eq:dual}) is to use better optimization algorithms that reduce the number of $(g_\gamma, \nabla g_\gamma)$ evaluations.

Eclipse~\cite{basu2020} uses the accelerated gradient descent (AGD) method~\cite{nesterov2004introductory} with a fixed step size, $1/L$ where $L$ is a global upper bound on the Lipschitz constant of $\nabla g_\gamma$ that is computed once at the beginning; this computation is also special for $A_i$ matrices with a diagonal structure. The cost is roughly equal to just a few $(g_\gamma, \nabla g_\gamma)$ evaluations and hence not worrisome. However, the bigger issue is that the conservative fixed step size means that the method needs a large number of steps to converge, with each step requiring one $(g_\gamma, \nabla g_\gamma)$ evaluation. The following points are important to note. (a) The bound on $L$ is inversely proportional to $\gamma$ and so, as $\gamma$ becomes small, $L$ becomes large, the fixed step size becomes extremely small and the Eclipse method becomes very slow. (b) Lipschitz constant values vary a lot in different parts of the
$(\gamma, \lambda)$ space. For efficient optimization, the right approach is to adapt the step size along the optimization path.

At each optimization iteration, a good optimization method will (a) select a good direction, (b) choose a starting step size, $\eta_0$, and, (c) start from $\eta_0$ and do efficient line search to obtain the final step size, $\eta$. To get a good $\eta_0$, we devise a heuristic method for estimating the Lipschitz constant.

{\bf Adaptive $\mathbf{L}$ estimation}
Let $H$ be the size of the history (number of previous iterations) we use to estimate the Lipschitz constant for the $t^{th}$ iteration. We use
\begin{equation}
    L_t= \max  \frac{||\nabla g(\lambda_s) - \nabla g(\lambda_{s-1}) ||}{|| \lambda_s - \lambda_{s-1} ||} \biggr\rvert_{s=t}^{t-H}
\end{equation}
The starting step size for the $t^{th}$ iteration, $\eta_0$ is then given by $\eta_0 = \eta_{min}$ if $t \leq H$; and, $\eta_0 = \min (1/L_t, \eta_{max})$ if $t > H$, where $\eta_{min}$ and $\eta_{max}$ are lower and upper bounds on the starting step size.
%We have bounds for min step size $(s_{min} = 1E-5)$ and max step size $(s_{max} = 0.1)$. 

For line search, the weak Wolfe bisection method~\cite{Burke2018LineSA} starting from $\eta_0$ is suitable for use with a traditional optimization algorithm. 

{\bf Projected Gradient Ascent (PGA)} For solving the constrained maximization problem (\ref{eq:dual}), the simplest method is to use the above adaptive $L$ estimation and line search ideas with projected gradient ascent, in which, at a given $\lambda_t$ with gradient $d_t = \nabla g_\gamma(\lambda_t)$, line search is done along the piecewise linear path, $\lambda(\eta) = \max (\lambda_t+\eta d_t, 0)$ where the $\max$ operation is applied component-wise. 

{\bf LBFGS-B} LBFGS-B~\cite{Byrd95alimited-memory} is an even better method is LBFGS-B, which is a specialized version of LBFGS for problems with bound constraints.

{\bf Experiment 1}
Choose a couple of datasets for which we know the true obj fun optimum, say a unit test problem or a decent sized problem that can be solved 
exactly using SCS. Plot the $\log (g_\gamma(\lambda_\gamma) - g_\gamma(\lambda_t))$ vs number of $g_\gamma$ evaluations. Show AGD-Eclipse, LBFGS-B and PGA as three curves on the same plot. Time to reach $10^-3*gdiff$ can also be shown.

{\bf Experiment 2} 
Take three $\gamma$ values - big to small - and show how difficult the problem solution becomes as $\gamma$ becomes small. We can study this for all three methods separately (e.g., for each method, one plot of $(g_\gamma(\lambda_\gamma) - 
g_\gamma(\lambda_t))$ vs number of $g$ evaluations that overlaps all 3 $\gamma$ solutions) and later decide how to organize the plots compactly. Time to reach $10^-3*gdiff$ can also be shown.

Write summary conclusions. We should not make any big novelty claim here except say that, the new choices give great improvements over Eclipse.



==> paper/qual.tex <==

\vspace{-0.2cm}
\section{Optimality and Infeasibility Detection}
\label{sec:optinfeas}

\def\PP{{\cal{P}}_1}

Real world large scale problems are usually run with limited computational resources and it is useful to find ways to stop the solution process early with some satisfactory guarantees of quality. In this section we give a few helpful tips for this.


\def\xtilde{\tilde{x}}
\def\dtilde{\tilde{dg}}
\def\xbar{\bar{x}}

{\bf Duality gap bound:} Suppose we are at some $\lambda$. In terms of the objective function $g_0(\lambda)$, we would like to know how close we are to optimality. Let $f^*$ denote the minimum objective function value of the primal (\ref{eq:main_problem}). By strong duality, $f^* = g_0^* = \min_{\lambda\ge 0} g_0(\lambda)$. Thus the duality gap, $d = f^* -g_0(\lambda)$. If $\xtilde$ is any feasible point for (\ref{eq:main_problem}) then by weak duality, $\dtil = c^T\xtilde - g_0(\lambda)$ satisfies $d \le \dtil$. But, how do we get a good $\xtilde$? We can take  $\xbar= \min_{x\in \C} (c + A^T\lambda)^T x$ (which is involved in the determination of $g_0(\lambda)$ and which possibly violates $Ax\le b$), and try to minimally alter it to obtain an $\xtilde$ that satisfies $Ax\le b$. There is no general method known in the literature to do this. Appendix~\ref{app:dgap} illustrates such an $\xtilde$ determination for one useful and popular class of $Ax\le b$ constraints.


%\subsection{Infeasible formulation}
%\label{subsec:qa_infeasible}

{\bf Infeasibility checking:}  
If the primal problem (\ref{eq:qp}) is infeasible, then $g_\gamma^* = \max_{\lambda\ge 0} g_\gamma(\lambda) = \infty$. For a given constraint type $\C_i$, it is easy to calculate a bound $B$ such that $\sum_i \max_{x_i} (c_i^Tx_i + \frac{\gamma}{2} x_i^Tx_i) \leq B$. Now, if the primal is feasible, then strong optimality implies that $g_\gamma^* \le B$. Thus, if, during the maximization, $g_\gamma > B$, then it means that the primal is infeasible. Appendix~\ref{app:infeas} %of the supplement~\cite{supplement}
gives a useful heuristic method to help fast infeasible detection.



==> paper/qualitative.tex <==
\section{Qualitative Analysis}
\label{sec:qualitative}

The evaluation in previous sections either leveraged the datasets with known solution or the datasets that can be handled by the baseline. The highest practical value of DualLip is the cases when neither is possible due to the scale of the problem. While DuaLip is guaranteed to converge given enough time (if the problem is feasible), the application may be constrained by available computational resources and algorithm is stopped early. In this scenario we need ways to estimate the quality of the solution. We give several recommendations for DuaLip practitioners that will help them better understand the behavior of the algorithm. We will cover the following topics: 1) detection of infeasible problem formulation, 2) dealing with infeasible primal solutions and estimation of the duality gap, and 3) evaluation against a naive yet useful baseline.

\subsection{Infeasible formulation}
\label{subsec:qa_infeasible}
The problem is infeasible if no points satisfy all the constraints. Having an infeasible formulation is common for large scale internet applications. For instance, user-item matching problem described in section~\ref{subsec:applications} can easily become infeasible with the equality simplex constraint $\sum_j x_{ij}=1$. This constraint requires to impress an item for every request, which becomes impossible if all eligible campaigns run out of budget. An infeasible primal has unbounded dual and as a result the optimization algorithm will never converge (see figure~\ref{fig:qa_infeasible}) and it is important to detect such situations. To establish infeasibility we can estimate the upper bound of the primal objective that is also an upper bound of the dual. If the dual objective gets above its upper bound the primal is infeasible. Estimation of the upper bound is problem-specific, for instance, an obvious upper bound for item matching problem can be obtained by selecting the worst\footnote{We formulate the primal as a minimization problem, and the $c_{ij}$ are negated costs, so the worst element would have the highest $c_ij$ value} item for each impression: $g^* \ge \sum_i \max_j c_{ij}$ (figure~\ref{fig:qa_infeasible}).

What do we do if the formulation is infeasible? One has to relax the formulation, usually the relaxation comes from the business requirements. For instance, we may be able to skip the impression if there are no items with the budget remaining or we may display items for free. Mathematically it is equivalent to relaxing the equality simplex constraint into inequality $\sum_j x_{ij}\le1$. The solution of such relaxation is also presented in figure~\ref{fig:qa_infeasible}. Unboundedness of the original dual is obvious when compared to the dual of the relaxed problem. Qualitative behavior of the dual does not prove the infeasibility (bound violation does) but it gives us an early sign of potential infeasibility much sooner than bound violation mathematically confirms it.

\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth, clip]{img/jobs-infeasible.pdf}}
\caption{Demonstration of infeasible formulation: unbounded dual function (solid red line) keeps increasing with time, compared to the dual function of a feasible relaxation (dotted green line) that plateaus at its maximum. The top horizontal line (dashed blue) represents the upper bound estimation for the dual. The dual violates the bound and it proves infeasibility.}
\label{fig:qa_infeasible}
\end{center}
\vskip -0.2in
\end{figure}

\subsection{Duality gap}
\label{subsec:qa_duality}
To evaluate the algorithm performance we need to compute the primal objective. In the optimal point the primal is equal to the dual $f^* = g^*$, but if we terminate early it is not the case. We compute the primal objective for a given $\lambda$ as $f(x(\lambda))$ via solving the projection problem \eqref{proj:eq1}. However, $x$ computed this way can be non-feasible for $\lambda\ne\lambda^*$ and the corresponding primal value is not a useful estimator of the objective. We suggest two approaches to address this problem: 1) derive a feasible solution from an infeasible one by projecting it to the feasible set or 2) penalize the objective if the constraints are violated. The amount of penalty is often known from the business requirements. For example, in a revenue maximization item matching problem with item-level budgets we can scale down $x_ij$ for items with budget violations until the problem is feasible. Alternatively we can penalize the objective by budget violations: $f^\tilde = cx - \sum_j \min(0, b_j - a_jx|)$ (possible because objective and constraints are expressed in the same units). For this problem both transformation of $x$ and penalization of objective yield the same result. We demonstrate it in figure~\ref{fig:qa_duality_gap}.

\begin{figure}[ht]
\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=\columnwidth, clip]{img/duality-gap.pdf}}
\caption{Visualization of the quality of the solution. The gap between dual and primal at transformed/feasible $x$ allows to estimate the potential of further objective improvement. The greedy baseline gives a reference point for estimating the magnitude of the gap. The baseline is built using using a greedy replay algorithm: each impression is assigned the best item with sufficient budget left, the budgets updated in real time.}
\label{fig:qa_duality_gap}
\end{center}
\vskip -0.2in
\end{figure}


\subsection{Simple baselines}
\label{subsec:qa_simbaseline}
In real applications it is important to evaluate the quality of the solution produced by an optimization algorithm against a simple and intuitive baseline. Very often, it is a greedy allocation algorithm with a set of business rules that ensure the constraints are satisfied. For example, for item matching problems the greedy solution would pick the best item with sufficient remaining budget and update the budget in real time. We show this baseline in figure~\ref{fig:qa_duality_gap}. The duality gap that characterizes the maximum unrealized improvement is contextualized in a comparison with the gain over the baseline.
